ESB: A Benchmark For Multi-Domain End-to-End Speech Recognition

Speech recognition applications cover a range of different audio and text distributions, with different speaking styles, background noise, transcription punctuation and character casing. However, many speech recognition systems require dataset-specific tuning (audio filtering, punctuation removal and normalisation of casing), therefore assuming a-priori knowledge of both the audio and text distributions. This tuning requirement can lead to systems failing to generalise to other datasets and domains. To promote the development of multi-domain speech systems, we introduce the End-to-end Speech Benchmark (ESB) for evaluating the performance of a single automatic speech recognition (ASR) system across a broad set of speech datasets. Benchmarked systems must use the same data pre- and post-processing algorithm across datasets - assuming the audio and text data distributions are a-priori unknown. We compare a series of state-of-the-art (SoTA) end-to-end (E2E) systems on this benchmark, demonstrating how a single speech system can be applied and evaluated on a wide range of data distributions. We find E2E systems to be effective across datasets: in a fair comparison, E2E systems achieve within 2.6% of SoTA systems tuned to a specific dataset. Our analysis reveals that transcription artefacts, such as punctuation and casing, pose difficulties for ASR systems and should be included in evaluation. We believe E2E benchmarking over a range of datasets promotes the research of multi-domain speech recognition systems. ESB is available at https://huggingface.co/esb.

==> 14app_errorcorrection.tex <==
Below we describe the annotation correction steps taken for each dataset.

\paragraph{LibriSpeech}
No annotation error corrections.

\paragraph{Common Voice} Many examples have incorrect trailing quotations marks, e.g \emph{"the cat sat on the mat."} instead of \emph{the cat sat on the mat.}, probably due to wrong transcription submissions. It does not make sense to wrap a standalone sentence that is considered without any context into quotation marks. In these cases, we strip the trailing quotation marks, leaving: \emph{the cat sat on the mat.}. Additionally double or triple quotation marks are corrected to single quotation marks (e.g. \emph{"""wait!""" they cried} $\rightarrow$ \emph{"wait!" they cried}) as double or triple quotation marks do not exist in the English language.

\paragraph{VoxPopuli}
No annotation error corrections.

\paragraph{TED-LIUM}
Transcriptions in the train set contain instances of the \emph{<unk>} token that are not present in the validation and test sets. We remove these tokens from the train set. Additionally, we correct incorrect leading spaces before apostrophes by collapsing spaced apostrophes into unspaced apostrophes (e.g. \emph{it 's} to \emph{it's}). We omit transcriptions labelled \emph{ignore\_time\_segment\_in\_scoring} from our evaluation by filtering them out.

\paragraph{GigaSpeech}
We remove official junk tokens (\emph{<sil>}, \emph{<music>}, \emph{<noise>}, \emph{<other>}) as they cannot be considered audio transcriptions, but rather elements useful for audio classification. We convert the spelled out punctuation to symbolic form (e.g. \emph{<comma>} $\rightarrow$ \emph{,}) since the speaker did not pronounce \emph{comma}, but instead the orthographic comma is meant.

\paragraph{Earnings-22}
We remove the official junk tokens (\emph{<crosstalk>}, \emph{<affirmative>}, \emph{<inaudible>}, \emph{<laugh>}).

Note on chunking:

\paragraph{SPGISpeech}
No annotation error corrections.

\paragraph{AMI}
Audio samples in the AMI meeting corpus vary from between 10 and 60 minutes in duration. We segment the audio samples according the the Kaldi \citep{Povey11_kaldi} recipe for AMI\footnote{https://github.com/kaldi-asr/kaldi/tree/master/egs/ami/s5b}; we split samples longer than X words at the time-stamps for punctuation to yield utterance of suitable length for training speech recognition systems.

\paragraph{SwitchBoard}
TODO (Patrick) need help here from Sanchit
Contains background noises / non-speech sounds denoted by square brackets, for example:
\begin{itemize}
    \item $\text{[noise]}$
    \item knock-knock [silence]
    \item who’s there [laughter]
\end{itemize}
Partially pronounced words, again denoted by square brackets. e.g.:
\begin{itemize}
    \item we love the w[ork] and involvement of the speech comm[unity]
    \item head to huggin[g] face dot co to find out m[ore]
\end{itemize}
Common alternate pronunciations, denoted by underscores, e.g.:
\begin{itemize}
    \item okay (pron. oh-kay) vs okay\_1 (pron. ’kay)
    \item Australia (pron. Australia) vs Australia\_1 (pron. ’straya)
\end{itemize}
Anomalous words, denoted by backslashes, e.g.: 
Angle braced words, that mark speech to someone, e.g.: <a\_aside>, <b\_aside>, <e\_aside>
Words containing laughter, e.g.: [laughter-because], [laughter-who], [laughter-now]
Coinages (made up / colloquial words), enclosed in curly braces e.g.: {alrighty}, {righty-ho}, {scammy}

We remove the background noises and non-speech sounds, as well as the square (resp. curly) brackets that denote partially pronounced words (resp. coinages), and the underscores that indicate alternate pronunciations:
\begin{itemize}
    \item knock-knock [silence] $\rightarrow$ knock-knock
    \item okay\_1, who's there $\rightarrow$ okay, who’s there
    \item we love the w[ork] and involvement of the speech comm[unity] $\rightarrow$ we love the work and involvement of the speech community
    \item {alrighty} [laughter], head to huggin[g] face dot co to find out m[ore] $\rightarrow$ alrighty, head to hugging face dot co to find out more
    \item it's [laughter-because] we want to find out maw/more $\rightarrow$ it's because we want to find out more
\end{itemize}

\paragraph{Fisher}

TODO: AMI (Patrick) -> no error correction here except converting <comma> to ,
TODO: CHiME-4 (Patrick) -> lots of converting <comma> to ,
